Inner Product Aware Quantization: Provably Fast, Accurate, and Adaptive Algorithms

Quantization is a fundamental tool used to compress datasets, neural network weights, and memory usage in a range of computational tasks. Many downstream applications of vector quantization perform inner products with arbitrary inputs. This motivates the study of inner product aware quantization schemes that approximately preserve inner products with unseen vectors -- in contrast to simply minimizing the mean-squared error. In this work, we formulate objectives that capture natural desiderata and develop adaptive and unbiased quantization methods that approximately preserve inner products with worst-case and average-case inputs. An analysis of these objectives shows a tight connection with the well-studied notion of Adaptive Stochastic Quantization (ASQ). We develop provably fast exact and approximate algorithms for our objectives. Our theoretical results inspire efficient practical algorithms that perform well across a variety of workload distributions. They also lead to practical algorithms for standard ASQ which are 2-10$\times$ faster than prior state-of-the-art methods while maintaining quality. These theoretical and empirical results contribute towards making adaptive quantization techniques more efficient and tractable in practical settings.

==> checklist.tex <==
% !TEX root = checklist-standalone.tex
\section*{NeurIPS Paper Checklist}


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}
    \item[] Justification: We provide theoretical and empirical evidence for every one of our claims throughout the paper. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A \answerNo{} or \answerNA{} answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{}
    \item[] Justification: See Section~\ref{sec: discussion} for a discussion of the limitations of our work. In all empirical evaluations, we clearly specify the type/distribution of inputs used.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper has no limitation while the answer \answerNo{} means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate ``Limitations'' section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that are not acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{}
    \item[] Justification: The full proofs of every theorem/lemma statement are provided in the appendices. We provide proof sketches for intuition in the main body. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

\item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{}
    \item[] Justification: In Section~\ref{sec: experimental-setup} we provide full details of the hardware on which our runtime experiments are conducted, and in Section \ref{sec:llm-expers} we fully detail the setup of our LLM quantization experiments. We provide the full details of all our empirical algorithms, the parameters with which they are run, and the data distributions/datasets on which they are run.    
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item If the paper includes experiments, a \answerNo{} answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and\slash or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{}
    \item[] Justification: The full code repository is available at\newline \texttt{https://github.com/nathanllww/Inner-Product-Aware-Quantization}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so \answerNo{} is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer) necessary to understand the results?
    \item[] Answer: \answerYes{}
    \item[] Justification: We specify all distributions used in our testing suite, algorithmic parameters, LLMs, and datasets. See plot captions throughout the paper. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{}
    \item[] Justification: All plots throughout the paper include error ranges indicating the $10$-$90$\% result quantiles. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The authors should answer \answerYes{} if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g., negative error rates).
        \item If error bars are reported in tables or plots, the authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{}
    \item[] Justification: See Section~\ref{sec: experimental-setup} for a full specification of the hardware used to run all our runtime experiments.  For our LLM quantization experiments, the accuracy results do not depend on the hardware used, and the full experimental setup can be found in Section~\ref{sec:llm-expers}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that did not make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{}
    \item[] Justification: Our results do not involve human subjects nor the potential for societal harm.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer \answerNo, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{}
    \item[] Justification: Our work addresses a foundational primitive found in many systems. It does not address a particular application. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that there is no societal impact of the work performed.
        \item If the authors answer \answerNA{} or \answerNo, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate Deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pre-trained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{}
    \item[] Justification: We do not release any data or models. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{}
    \item[] Justification: We use and acknowledge the code and data of \cite{GKMNSS17} and \cite{carlson2025newpairgloves} respectively.
        Our use of Qwen3.5-4B is allowed under the Apache 2.0 license of the weights.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{}
    \item[] Justification: We do not release any assets with this submission. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset\slash code\slash model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{}
    \item[] Justification: Our work does not involve human subjects. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{}
    \item[] Justification: Our work does not involve human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does \emph{not} impact the core methodology, scientific rigor, or originality of the research, declaration is not required.
    \item[] Answer: \answerYes{}
    \item[] Justification: We used LLM tools to improve the presentation of this work, and to improve the proof of Theorem \ref{thmt@@ADVApproxAlg}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy in the NeurIPS handbook for what should or should not be described.
    \end{itemize}

\end{enumerate}


==> intro.tex <==
\section{Introduction}

Vector quantization is an incredibly important tool that is central to space and runtime optimization in a wide variety of computational applications. Most notably, it is a prominent method used to compress datasets, neural network weights, and memory usage in a range of computational tasks.

% That is, given a vector $w \in \R^d$, we'd like to quantize it to a vector $\bwh \in Q^d$ where $|Q| = s \ll d$ such that for every input vector $x \in \R^d$, $\la \bwh, x\ra \approx \la w, x \ra$.

Formally, we define vector quantization as follows.
Let $w \in \R^d$ and let $Q \subset \R$ be a set of \emph{quantization values} such that $|Q| = s \ll d$.
% Vector $w$ can be \emph{quantized} via some \emph{rounding distribution} $\calD$ (which possible depends on $w$) with $\text{Supp}(\calD) \subseteq Q^d$ that rounds every entry of $w$ to an element in $Q^d$
Vector $w$ can be \emph{quantized} via some \emph{rounding distribution} $\calD$ with $\text{Supp}(\calD) \subseteq Q^d$. 

% That is, $\bwh \sim \calD$\footnote{We use boldface to denote random variables} is such that $\bwh \in Q^d$.

An important consideration of this work is the emphasis on \emph{unbiased} and \emph{adaptive} quantization schemes. Formally, a quantization scheme is \emph{unbiased}\footnote{Note that any deterministic rounding distribution other than the identity is necessarily biased} if $\E_{\bwh \sim \calD}[\bwh] = w$. An adaptive quantization scheme $(Q, \calD)$ is one where both $Q$ and $\calD$ may depend on $w$ so as to optimize an objective function of choice.

Previous work on unbiased quantization gave schemes that are non-adaptive or very weakly adaptive \cite{alistarh2017qsgd, ramezani2021nuqsgd}.
Some works designed schemes suited to optimize a worst-case vector $w$, while others used only superficial properties of the vectors such as their norm or aspect ratio.
On the other hand, some solutions designed schemes for vectors $w$ coming from some pre-specified distribution.
For example, much real-world data is known to loosely follow Log-Normal \cite{chmiel2020neural} or Normal \cite{banner2019post, ye2020accelerating} distributions.
Prior work has also shown that the weights in deep layers of neural networks often follow a sub-Weibull distribution \cite{vladimirova2018bayesian}.

Previous work on non-adaptive/weakly adaptive quantization schemes such as Round-To-Nearest, QSGD \cite{alistarh2017qsgd}, and NUQSGD \cite{ramezani2021nuqsgd} show poor performance when evaluated under the Mean Squared Error ($\MSE$) objective (see Figure 1 of \cite{ben2024optimal}).
In contrast, a prominent line of work on \emph{adaptive stochastic quantization} (ASQ) by \cite{ben2024optimal, ZLKALZ17} studies adaptive and unbiased quantization schemes to optimize mean-squared error ($\MSE$). 

In particular, they consider the simple rounding distribution known as \emph{stochastic quantization}. Stochastic quantization of a vector $w \in \R^d$ to a quantization set $Q$ is the procedure of rounding each entry $w_i$ of $w$ to $\{ \widown(Q), \wiup(Q) \}$, where $\wiup(Q) := \min \{q \in Q: w_i \leq q\}$ and $\widown(Q) := \max \{ q \in Q: w_i \geq q \}$, in an independent and unbiased manner. The unique such rounding scheme rounds to $\widown$ with probability $p^{\ardo} =  (\wiup - w_i)/(\wiup - \widown)$ and to $\wiup$ with probability $p^{\arup} = (w_i - \widown)/(\wiup - \widown)$, which results in $\E[\bwh] = w$ and $\Var[\bwh] = (\wiup - w_i)(w_i - \widown)$. 
% Given a scalar $w \in [\wdown{}, \wup{}]$, Stochastic quantization (SQ) is the procedure that rounds $w$ to $\bwh \in \{ \wdown{}, \wup{} \}$ in an unbiased manner. That is, the procedure rounds to $\wdown{}$ with probability $p^{\scriptstyle\scriptstyle \downarrow} =  (\wup{} - w)/(\wup{} - \wdown{})$ and to $\wup{}$ with probability $p^{\arup} = (w - \wdown{})/(\wup{} - \wdown{})$ so that
% \bnote{I think we should maybe define relative to a full quantization set; while this works, it's a bit out of the way to say ``first suppose there's only two options.  now do the same thing but with the nearest elements of $Q$''? but this explanation is also quite clear, so I see an arg for keeping as is too}
% \begin{align*}
%     \E[\bwh] = p^{\ardo} \cdot \wdown{} + p^{\arup} \cdot \wup{} = \frac{\wup{} - w}{\wup{} - \wdown{}} \cdot \wdown{} + \frac{w - \wdown{}}{\wup{} - \wdown{}} \cdot \wup{} = w
% \end{align*}
% Observe that stochastic quantization is the unique unbiased distribution in such a setting. The variance is given by
% \begin{align*}
% \Var[\bwh] = \E[(\bwh - w)^2] = p^{\ardo} \cdot (\wdown{} - w)^2 + p^{\arup} \cdot (\wup{} - w)^2 = (\wup{} - w)(w - \wdown{})
% \end{align*}

 We let $\smash \dasq(w, Q)$\footnote{When it is clear from the context, we write $\dasq$ as shorthand.} denote the stochastic quantization rounding distribution for a particular $(w, Q)$ pair. Similarly, we let $\smash \VarASQ(w_i, Q) := (\wiup - w_i)(w_i - \widown)$ denote the variance of a particular coordinate $w_i$ for a pair $(w, Q)$. 

 Then, the optimization problem is to find the quantization set $Q \subset \R$ with target size $s$ that minimizes the mean squared error
 $$\MSE(\bwh,w) \triangleq \E \left[~\norm{\bwh - w}_2^2 \right] = \sum_{i \in [d]} \VarASQ(w_i, Q) = \sum_{i \in [d]} (\wiup - w_i)(w_i - \widown)$$
\cite{ZLKALZ17} first gave an algorithm to find the optimal adaptive quantization set $Q$ using dynamic programming with runtime and memory $O(d^2 s)$. This was later improved by \cite{ben2024optimal} to $O(d \log d + ds)$ runtime and $O(ds)$ space by employing fast algorithms for matrix searching in totally monotone matrices \rnote{ref: smawk}. 

% objective provides algorithms that convincingly outperform existing counterparts \cite{ZLKALZ17}.
% \bnote{I think this sentence is mixing algorithms and objectives a bit?}



% \onote{maybe we should add a ``our contributions'' subsection header at this point?}
% \rnote{More generally, I think this intro section might benefit from a bit more structure; it's a bit in a stream rn which could make it hard for a reader to jump to one part or another}

\subsection{Inner Product Aware Quantization}

The widespread use of vector quantization for tasks such as neural network weight compression and vector search illustrates that the success of many important modern downstream tasks depends on quantization methods that approximately preserve inner products. This heavily motivates the need for \emph{inner product aware} quantization methods.
That is, one should expect the performance quality of salient downstream tasks to be enhanced if the quantized vectors preserve their inner products with arbitrary input vectors. See Section \ref{sec: motivation} for more in-depth discussion and evidence for the benefit of inner product aware quantization.

In this work, we study inner product aware quantization both from theoretical and empirical lenses.
On the theoretical side, we formulate concrete objectives that capture natural desiderata for inner product preserving quantization.
We design provably fast exact and approximation algorithms for these objectives and prove bounds on their solution quality (see Section \ref{sec: theoretical-results}).
On the empirical side, we implement theory-inspired heuristics and show that they significantly outperform existing implementations in efficiency and quality.
Through these heuristics, we also give much faster algorithms than those of \cite{ben2024optimal} for traditional ASQ.
See Section \ref{sec: empirical-results} for our main empirical contributions and performance on approximate nearest neighbor benchmarks.

% More precisely, an informal statement of the central question of this work is the following: given a vector $w \in \R^d$, can we efficiently find a quantization set $Q$ with $|Q| = s \ll d$ and \emph{rounding distribution} $\calD$ with $\text{Supp}(\calD) \subseteq Q^d$ such that for an input vector $x \in \R^d$, $\la \bwh, x\ra \approx \la w, x \ra$ with high probability over a draw of $\bwh \sim \calD$?
% \bnote{I think we can remove the sentence?  it seems like we've already mentioned this, just not in symbols?}



In full generality, we wish to jointly optimize over the tuple $(Q, \calD)$ according to some to-be-defined objective function.
As a first step, we consider the simpler goal of fixing a quantization set $Q$ and optimizing for the best corresponding rounding distribution.
The $\objth$ (Definition \ref{def: wddv}) and $\objf$ (Definition \ref{def: addv}) objectives capture this question for inner product preservation for a (1) worst-case input vector $x \in \R^d$ and (2) average-case input vector $x \sim \calX$ for some known input distribution $\calX$.
% \bnote{throughout the paper, when using this (1), (2) sentence notation, we sometimes use roman and sometimes arabic numerals.  should unify; this can be an LLM task}

% \bnote{we've sort of mentioned the stochastic quantization/ASQ definition a few times already; maybe moving this definition up would be helpful?}
We show in Theorem \ref{thm:objective-three-optimal-rounding} that \emph{stochastic quantization} turns out to be optimal for $\objth$ (minimizing the worst-case variance)! When considering $\objf$, however, the situation is more challenging: in Theorem \ref{thm:addv-np-hard}, we show that computing the optimal distribution for $\objf$ (minimizing average-case variance) is NP-Hard.
Given the result of Theorem \ref{thm:objective-three-optimal-rounding}, it is thus natural to fix the rounding distribution $\dasq$ both in the worst and average case settings. Then, the optimization is over quantization sets $Q$. 
% The thrust of this work is in the second direction of the joint optimization over $(Q, \calD)$:
% given a rounding distribution $\dasq$, we develop efficient algorithms to find optimal and approximate quantization sets that inherently preserve inner products.
% Thus, much of this work considers the fixed rounding distribution $\dasq(w, Q)$ and optimizes the quantization set $Q$
% \bnote{I think we should clearly delineate the development of algorithms and objectives; the previous sentence is my changed version but I also left the old commented out as it's a somewhat substantive change}
We formulate the following two corresponding objectives, and then design fast algorithms for them (the algorithmic results are outlined in Section \ref{sec: theoretical-results}).

% \newpage


% Throughout the paper, given a vector $w$, we write $\widown(Q)$ to be the largest element of $Q$ less than or equal to $w_i$ and $\wiup(Q)$ as the smallest element larger than $w_i$.

% \begin{definition}[Standard rounding distribution]
%     For a vector $w\in \mathbb{R}^{d}$ and a set $Q\subset \mathbb{R}$, we define the standard ASQ rounding distribution $\dasq(w,Q)$ to be the distribution over $Q^{d}$ where for $\bwh\sim \dasq(w,Q)$ and all $i\in [d]$, $\bwh_i=\widown(Q)$ with probability $(\wiup(Q)-w_i)/(\wiup(Q)-\widown(Q))$ and $\bwh_i=\wiup(Q)$ with probability $(w_i-\widown(Q))(\wiup(Q)-\widown(Q))$.
% \end{definition}

% It is useful to have a notion of variance of a single value $w_i$ when rounded according to a set $Q$ and $\dasq(w,Q)$.
% \begin{definition}
%     For a vector $w\in \mathbb{R}^d$ and a set $Q\subset \mathbb{R}$, let
%     \[\varasq(w_i, Q) = \var_{\bwh\sim \dasq(w,Q)}[\bwh_i] = (w_i - \widown(Q))(\wiup(Q) - w_i).\]
%     % where $\widown(Q)$ is the largest element of $Q$ less than or equal to $w_i$ and $\wiup(Q)$ is the smallest element of $Q$ larger than $w_i$.
% \end{definition}

\begin{definition}[Maximum Directional Variance ($\objo$)]
    For a vector $w\in \mathbb{R}^{d}$ and target quantization set size $s \in \N$, we define
    \[\objo(w,s) \triangleq \min_{Q \subset \R: |Q| \leq s} \max_{x\in \mathbb{R}^{d}: \|x\|_2 \leq 1} \var_{\bwh\sim \dasq(w,Q)}[\langle \bwh,x \rangle]\]
\end{definition}
For a fixed quantization set $Q$, we write $$\objo(w, Q) \triangleq \max_{x\in \mathbb{R}^{d}: \|x\|_2 \leq 1} \var_{\bwh\sim \dasq(w,Q)}[\langle \bwh,x \rangle]$$ to denote its $\objo$ objective cost. $\objo$ has a simple combinatorial structure: in particular, observe that
\begin{align*}
    \objo(w, Q) &= \max_{x\in \mathbb{R}^{d}: \|x\|_2 \leq 1} \left[ \var_{\bwh\sim \dasq(w,Q)}[\langle \bwh,x \rangle] \right] \\
    &= \max_{x\in \mathbb{R}^{d}: \|x\|_2 \leq 1} \left[ \sum_{i=1}^d x_i^2 \var_{\bwh\sim \dasq(w,Q)}[\bwh_i] \right] \tag{Independence of $\dasq$} \\
    &= \max_{j\in [d]} \varasq(w_j, Q).
\end{align*}
% \bnote{is ``input vector'' the best name for $x$?}
So, the worst-case input vector $x$ is the standard unit basis vector $e_i$ where $i$ is such that $\VarASQ[\bwh_i]$ is maximized. In practice, however, input vectors $x$ are often not worst-case, and instead come from some known (or estimated) distribution. As such, we also consider optimizing to minimize the average variance over some (known) distribution of vectors $x$.
% \begin{observation}
%     For any $w\in \mathbb{R}^{d}$ and $Q \subset \mathbb{R}$,
%     \[
%         \objo(w,Q) = \max_{i\in [d]} \varasq(w_i, Q).
%     \]
% \end{observation}
% \begin{proof}
%     From the definition of inner products and the fact that $\bwh_i$ are independent, we have for all $x\in \mathbb{R}^{d}$ with $\|x\|_2=1$,
%     \begin{align*}
%         &\var_{\bwh\sim \dasq(w,Q)}[\langle \bwh,x \rangle] = \var_{\bwh\sim \dasq(w,Q)}\left[\sum_{i=1}^d \bwh_i x_i\right] = \sum_{i=1}^d x_i^2 \var_{\bwh\sim \dasq(w,Q)}[\bwh_i]\\
%         =&\sum_{i=1}^d x_i^2 \varasq(w_i, Q)\leq \max_{j\in [d]} \varasq(w_j, Q) \sum_{i=1}^d x_i^2= \max_{j\in [d]} \varasq(w_j, Q).
%     \end{align*}
%     Moreover, this upper bound is achieved by the vector $x$ which is $1$ in the coordinate $i$ which achieves the maximum and $0$ elsewhere, and thus $\objo(w,Q) = \max_{i\in [d]} \varasq(w_i, Q)$.
% \end{proof}

% \onote{avoid contractions (again something the LLM can also filter out); reworded this sentence anyway but leaving commented out for prosterity and leaving this comment for our note}
% In practice, however, we oftentimes \bnote{\sout{don't}} expect to encounter the worst-case and would prefer to develop algorithms tailored to the specific data distribution we expect to see.
% In particular, if the input vectors $x$ are known to be drawn from some distribution $\calX$, we define the Average Directional Variance ($\objt$) objective as a generalization of $\objo$. Note that we use $\dasq$ as the rounding distribution.
\begin{definition}[Average Directional Variance ($\objt$)]
    For a vector $w\in \mathbb{R}^{d}$, target quantization set size $s \in \N$, and input distribution $\calX$ over $\mathbb{R}^{d}$, define
    \begin{align}
        \objt_{\calX}(w, s) \triangleq \min_{Q \subset \R: |Q| \leq s} \E_{\bx \sim \calX} \left[\VarASQ \left[ \la \bwh, \bx \ra \right] \right]
    \end{align}
\end{definition}
Note that, with $\lambda_i \triangleq \E_{\bx \sim \calX} [\bx_i^2]$, for a fixed quantization set $Q$, we write 
\begin{align*}
    \objt_{\calX}(w,Q) \triangleq \E_{\bx\sim \calX}[\var_{\bwh\sim \dasq(w,Q)}[\langle \bwh,\bx \rangle]] = \sum_{i=1}^d \lambda_i \cdot \varasq[\bwh_i]
\end{align*}
to denote its $\objt$ cost. The $\objt$ objective turns out to have a familiar structure. 
\begin{align*}
    \min_{Q \subset \R: |Q| \leq s} \E_{\bx \sim \calX} \left[\VarASQ \left[ \la \bwh, \bx \ra \right] \right] &= \min_{Q \subset \R: |Q| \leq s} \E_{\bx \sim \calX} \left[ \sum_{i \in [d]} \bx_i^2 \cdot \VarASQ[\bwh_i] \right] \\
    &= \min_{Q \subset \R: |Q| \leq s} \sum_{i \in [d]} \lambda_i \cdot \VarASQ[\bwh_i]
    % &= \min_{Q \subset \R: |Q| \leq s} \sum_{i \in [d]} \lambda_i \cdot (\wiup(Q) - w_i)(w_i - \widown(Q))
\end{align*}
This can be interpreted as a weighted $\MSE$ objective function! We note that this connection between quantization for average-case inner product preservation and the problem of stochastic quantization under the weighted $\MSE$ objective provides a theoretical justification for the empirical success of Adaptive Stochastic Quantization for downstream applications in ML and vector search.


% \bnote{this is defining $\lambda_i$ after first use?}
% \ignore{Moreover, it is easy to see that for the purposes of constructing an optimal quantization set, it is equivalent to solve the optimization problem over the normalized weights $\lambda_i' \triangleq \lambda_i / \smash \sum_{i \in [d]} \lambda_i$. This is because the minimizing argument remains unchanged after normalization by a constant.}

% As long as distribution $\calX$ has finite marginal second moments, objective $\objt$ is well-defined.
% \bnote{I think it's well-defined even in the infinite variance case?  The objective is just either $\infty$ or 0 on the marginals with infinite variance.}
% We let $\Gamma$ denote the set of distributions over $\R^d$ with finite marginal second moments, and consider $\calX \in \Gamma$ for the entirety of the paper.






    % For a vector $w\in \mathbb{R}^{d}$ and a set $Q\subset \mathbb{R}$, we define
    % \[\objt(w,Q)=\sum_{i=1}^d \varasq(w_i, Q).\]
    % We usually also consider a weighted version of this objective, where we have a weight vector $\alpha\in \mathbb{R}^d$ and define
    % \[\objt_\alpha(w,Q)=\sum_{i=1}^d \alpha_i\cdot \varasq(w_i, Q).\]
    % We define $\objt_\alpha(w,s)$ to be the smallest value of $\objt_\alpha(w,Q)$ over all sets $Q$ of size at most $s$.
    % \bnote{When clear from context, we will omit the subscript $\alpha$ and simply write $\objt(w,Q)$ and $\objt(w,s)$.}
    % \bnote{{\footnotesize NLW:} Do we actually do this?}

% \begin{definition}[$\objth$, best worst-case rounding scheme]
%     \label{def:wddv}
%     For a vector $w\in \mathbb{R}^{d}$ and a set $Q\subset \mathbb{R}$, let $\Omega$ be the space of all distributions over $Q^{d}$ which are unbiased with respect to $w$, i.e.~$\mu(\calD) = w$ for all $\calD\in \Omega$.
%     Then, we define
%     \[\objth(w,Q)=\argmin_{\calD\in \Omega}\max_{x\in \mathbb{R}^{d}}\var_{\bwh\sim \calD}[\langle \bwh,x \rangle].\]
%     \gnote{Should the min be an argmin, i.e.~the distribution, or min, the value of the objective?}
% \end{definition}

% \begin{definition}[$\objf$, best distribution-dependent rounding scheme]
%     For a vector $w\in \mathbb{R}^{d}$ and a set $Q\subset \mathbb{R}$, let $\Omega$ be the space of all distributions over $Q^{d}$ which are unbiased with respect to $w$, i.e.~$\mu(\calD) = w$ for all $\calD\in \Omega$.
%     Given a distribution $\calX$ over $\mathbb{R}^{d}$, we define
%     \[
%         \objf(w,Q,\calX)=\argmin_{\calD\in \Omega}\E_{\bx\sim \calX}[\var_{\bwh\sim \calD}[\langle \bwh,\bx \rangle]].
%     \]
% \end{definition}



% One of the most important downstream tasks performed on high-dimensional vectors when doing RAG or Neural Network computations is inner product computations.
% Thus, a desirable property of any quantization method is to \textit{approximately} preserve the rounded vector's inner products with input vectors.
% In this section, we formalize this problem with two natural objectives that capture these desiderata.
% In this setting, we consider a fixed quantization set $Q$ or grid where vectors must round.
% Then, we wish to find an optimal \textit{rounding scheme} to $Q$.
% The rounding scheme will be a distribution $\calD$ with the property that $\text{supp}(\calD) \subseteq Q^d$.
% Naturally, $\calD$ is allowed to depend on $Q$.
% Importantly, we also allow $\calD$ to depend on $w$ (i.e. $\calD$ is allowed to be adaptive). The worst-case objective is defined as follows.
% \begin{align}
%     \objth(w, Q) \triangleq \min_{\text{Rounding schemes } \calD} \max_{x : \norm{x}_2 \leq r} \Var_{\buh \sim \calD}[\la \buh, x \ra] \\
%     \text{ subject to }
% \, \forall x \, \, \E_{\buh \sim \calD}[\la \buh, x \ra] = \la w, x \ra \notag
% \end{align}
% We define an analogous \emph{average-case} objective when the inputs $x$ are known to come from a distribution $\calX$.
% \begin{align}
%     \objf_{\calX}(w, Q) \triangleq \min_{\text{Rounding schemes } \calD} \E_{x \sim \calX} \left[ \Var_{\buh \sim \calD}[\la \buh, x \ra] \right] \\
%     \text{ subject to }
% \, \forall x \in \text{supp}(\calX) \, \, \E_{\buh \sim \calD}[\la \buh, x \ra] = \la w, x \ra \notag
% \end{align}











==> krish-intro.tex <==
\section*{Adaptive Stochastic Quantization: Provably Fast and Accurate Algorithms for Inner-Product Preservation}

\section{Krish's Introduction}

Vector quantization is an incredibly important tool that is central to space and runtime optimization in a wide variety of computational applications. \rnote{add examples!}

% That is, given a vector $w \in \R^d$, we'd like to quantize it to a vector $\bwh \in Q^d$ where $|Q| = s \ll d$ such that for every input vector $x \in \R^d$, $\la \bwh, x\ra \approx \la w, x \ra$.

Formally, we define vector quantization as follows.
Let $w \in \R^d$ and let $Q \subset \R$ be a set of \emph{quantization values} such that $|Q| = s \ll d$.
% Vector $w$ can be \emph{quantized} via some \emph{rounding distribution} $\calD$ (which possible depends on $w$) with $\text{Supp}(\calD) \subseteq Q^d$ that rounds every entry of $w$ to an element in $Q^d$
Vector $w$ can be \emph{quantized} via some \emph{rounding distribution} $\calD$ with $\text{Supp}(\calD) \subseteq Q^d$. An important consideration of this work is the emphasis on \emph{unbiased} and \emph{adaptive} quantization schemes. A quantization scheme is unbiased\footnote{Note that any deterministic rounding distribution other than the identity is necessarily biased} if $\E_{\bwh \sim \calD}[\bwh] = w$. An adaptive quantization scheme $(Q, \calD)$ is one where both $Q$ and $\calD$ may depend on $w$. 

Previous work gave schemes that are non-adaptive \cite{zandieh2025turboquant} or very weakly adaptive. Schemes such as QSGD \cite{alistarh2017qsgd} and NUQSGD \cite{ramezani2021nuqsgd} only use superficial properties of the vectors such as their norm or aspect ratio. Some works \cite{} designed schemes suited to optimize a worst-case vector $w$, leaving room for improvement on average-case inputs. On the other hand, some solutions designed schemes for vectors $w$ coming from some pre-specified distribution. For example, much real-world data is known to loosely follow Log-Normal \cite{chmiel2020neural} or Normal \cite{banner2019post, ye2020accelerating} distributions. Prior work has also shown that the weights in deep layers of neural networks often follow a sub-Weibull distribution \cite{vladimirova2018bayesian}. Even still, other work on schemes such as Round-To-Nearest provide biased quantization. 

In contrast, a prominent line of work on \emph{adaptive stochastic quantization} (ASQ) by \cite{ben2024optimal, ZLKALZ17} studies adaptive and unbiased quantization schemes. It has been shown that many biased and/or non-adaptive/weakly adaptive quantization schemes perform poorly in comparison. In the literature, the quality of quantization is often measured using the mean-squared error
$$\MSE(\bwh,w) \triangleq \E \left[~\norm{\bwh - w}_2^2 \right]$$ 

While a reasonable and useful metric, modern downstream applications of quantization motivate the need for new objectives. 
The widespread use of vector quantization for tasks such as neural network weight compression and vector search illustrates that the success of many important modern downstream tasks depends on quantization methods that approximately preserve inner products. We introduce the notion of \emph{inner-product aware} quantization that, roughly speaking, aims to preserve inner products $\la \bwh, x\ra \approx \la w, x\ra$ with high probability. Because we are considering unbiased rounding distributions $\calD$, maximizing the probability that $\la \bwh, x \ra \approx \la w, x \ra$ can be achieved by minimizing the \emph{directional} variance\footnote{Variance of $\bwh$ along direction $x$} $\Var_{\bwh \sim \calD}[\la \bwh, x \ra]$.

We consider a well-studied and fundamental rounding scheme known as \emph{stochastic quantization} (see preliminaries in section \ref{sec: prelims} for the formal definition and theoretical justification of this choice) and define suitable objectives that capture these natural desiderata.  We let $\smash \dasq(w, Q)$\footnote{When it is clear from the context, we write $\dasq$ as shorthand.} denote the stochastic quantization rounding distribution for a particular $(w, Q)$ pair. With the rounding distribution $\dasq$ fixed, the optimization is over the best quantization set $Q$ to minimize the variance of the (1) worst-case inner product and (2) average-case inner product. 

\begin{definition}[Maximum Directional Variance ($\objo$)]\label{def: mdv}
    For a vector $w\in \mathbb{R}^{d}$ and target quantization set size $s \in \N$, we define
    \[\objo(w,s) \triangleq \min_{Q \subset \R: |Q| \leq s} \max_{x\in \mathbb{R}^{d}: \|x\|_2 \leq 1} \var_{\bwh\sim \dasq(w,Q)}[\langle \bwh,x \rangle]\]
\end{definition}

In practice, however, input vectors $x$ are often not worst-case, and instead come from some known (or estimated) distribution. As such, we also consider optimizing to minimize the average variance over some (known) distribution of vectors $x$.

\begin{definition}[Average Directional Variance ($\objt$)] \label{def: adv}
    For a vector $w\in \mathbb{R}^{d}$, target quantization set size $s \in \N$, and input distribution $\calX$ over $\mathbb{R}^{d}$, define
    \begin{align}
        \objt_{\calX}(w, s) \triangleq \min_{Q \subset \R: |Q| \leq s} \E_{\bx \sim \calX} \left[\VarASQ \left[ \la \bwh, \bx \ra \right] \right]
    \end{align}
\end{definition}

In this work, we study inner-product aware quantization both from theoretical and empirical lenses.
On the theoretical side, we design provably fast exact and approximation algorithms for these objectives and prove bounds on their solution quality (see Section \ref{sec: theoretical-results}). \rnote{We don't talk about $\objth$ and $\objf$ here...} On the empirical side, we implement theory-inspired heuristics and show that they significantly outperform existing implementations in efficiency and quality. As shown in Section \ref{sec: prelims}, the $\objt$ objective turns out to be the weighted version of $\MSE$. Thus, our fast empirical algorithms for $\objt$ directly give much faster algorithms than those of \cite{ben2024optimal} for traditional ASQ. See Section \ref{sec: empirical-results} for our main empirical contributions and performance on approximate nearest neighbor benchmarks.
% . That is, one should expect the performance quality of salient downstream tasks to be enhanced if the quantized vectors preserve their inner products with arbitrary input vectors. See Section \ref{sec: motivation} for more in depth discussion and evidence for the benefit of inner-product aware quantization.




 


% \subsection{Inner-Product Aware Quantization}

% The widespread use of vector quantization for tasks such as neural network weight compression and vector search illustrates that the success of many important modern downstream tasks depends on quantization methods that approximately preserve inner products. This heavily motivates the need for \emph{inner-product aware} quantization methods.
% That is, one should expect the performance quality of salient downstream tasks to be enhanced if the quantized vectors preserve their inner products with arbitrary input vectors. See Section \ref{sec: motivation} for more in depth discussion and evidence for the benefit of inner-product aware quantization.

% In this work, we study inner-product aware quantization both from theoretical and empirical lenses.
% On the theoretical side, we formulate concrete objectives that capture natural desiderata for inner-product preserving quantization.
% We design provably fast exact and approximation algorithms for these objectives and prove bounds on their solution quality (see Section \ref{sec: theoretical-results}).
% On the empirical side, we implement theory-inspired heuristics and show that they significantly outperform existing implementations in efficiency and quality.
% Through these heuristics, we also give much faster algorithms than those of \cite{ben2024optimal} for traditional ASQ.
% See Section \ref{sec: empirical-results} for our main empirical contributions and performance on approximate nearest neighbor benchmarks.

% More precisely, an informal statement of the central question of this work is the following: given a vector $w \in \R^d$, can we efficiently find a quantization set $Q$ with $|Q| = s \ll d$ and \emph{rounding distribution} $\calD$ with $\text{Supp}(\calD) \subseteq Q^d$ such that for an input vector $x \in \R^d$, $\la \bwh, x\ra \approx \la w, x \ra$ with high probability over a draw of $\bwh \sim \calD$?
% \bnote{I think we can remove the sentence?  it seems like we've already mentioned this, just not in symbols?}

\subsection{Preliminaries} \label{sec: prelims}

\paragraph{Adaptive Stochastic Quantization.} \emph{Stochastic quantization} of a vector $w \in \R^d$ to a quantization set $Q$ is the procedure of rounding each entry $w_i$ of $w$ to $\{ \widown(Q), \wiup(Q) \}$, where $\wiup(Q) := \min \{q \in Q: w_i \leq q\}$ and $\widown(Q) := \max \{ q \in Q: w_i \geq q \}$, in an independent and unbiased manner. The unique such rounding scheme rounds to $\widown$ with probability $p^{\ardo} =  (\wiup - w_i)/(\wiup - \widown)$ and to $\wiup$ with probability $p^{\arup} = (w_i - \widown)/(\wiup - \widown)$, which results in $\E[\bwh] = w$ and $\Var[\bwh] = (\wiup - w_i)(w_i - \widown)$. 
% Given a scalar $w \in [\wdown{}, \wup{}]$, Stochastic quantization (SQ) is the procedure that rounds $w$ to $\bwh \in \{ \wdown{}, \wup{} \}$ in an unbiased manner. That is, the procedure rounds to $\wdown{}$ with probability $p^{\scriptstyle\scriptstyle \downarrow} =  (\wup{} - w)/(\wup{} - \wdown{})$ and to $\wup{}$ with probability $p^{\arup} = (w - \wdown{})/(\wup{} - \wdown{})$ so that
% \bnote{I think we should maybe define relative to a full quantization set; while this works, it's a bit out of the way to say ``first suppose there's only two options.  now do the same thing but with the nearest elements of $Q$''? but this explanation is also quite clear, so I see an arg for keeping as is too}
% \begin{align*}
%     \E[\bwh] = p^{\ardo} \cdot \wdown{} + p^{\arup} \cdot \wup{} = \frac{\wup{} - w}{\wup{} - \wdown{}} \cdot \wdown{} + \frac{w - \wdown{}}{\wup{} - \wdown{}} \cdot \wup{} = w
% \end{align*}
% Observe that stochastic quantization is the unique unbiased distribution in such a setting. The variance is given by
% \begin{align*}
% \Var[\bwh] = \E[(\bwh - w)^2] = p^{\ardo} \cdot (\wdown{} - w)^2 + p^{\arup} \cdot (\wup{} - w)^2 = (\wup{} - w)(w - \wdown{})
% \end{align*}

 We let $\smash \dasq(w, Q)$\footnote{When it is clear from the context, we write $\dasq$ as shorthand.} denote the stochastic quantization rounding distribution for a particular $(w, Q)$ pair. Similarly, we let $\smash \VarASQ(\bwh_i, Q) := (\wiup - w_i)(w_i - \widown)$ denote the variance of a particular coordinate $i$ for a pair $(w, Q)$. The mean squared error under stochastic quantization is then
 $$\MSE(\bwh,w) \triangleq \E \left[~\norm{\bwh - w}_2^2 \right] = \sum_{i \in [d]} \VarASQ(w_i, Q) = \sum_{i \in [d]} (\wiup - w_i)(w_i - \widown)$$

 
 

\paragraph{Inner-Product Aware Quantization. } Here, we provide a theoretical justification for the choice of $\dasq$ as the rounding distribution. In full generality, the problem of quantization asks to jointly optimize over the tuple $(Q, \calD)$ so as to optimize some objective function. As a first step, we consider the simpler goal of fixing a quantization set $Q$ and optimizing for the best corresponding rounding distribution. The $\objth$ (Definition \ref{def: wddv}) and $\objf$ (Definition \ref{def: addv}) objectives capture this question for inner product preservation for a (1) worst-case input vector $x \in \R^d$ and (2) average-case input vector $x \sim \calX$ for some known input distribution $\calX$.
% \bnote{throughout the paper, when using this (1), (2) sentence notation, we sometimes use roman and sometimes arabic numerals.  should unify; this can be an LLM task}

% \bnote{we've sort of mentioned the stochastic quantization/ASQ definition a few times already; maybe moving this definition up would be helpful?}
We show in Theorem \ref{thm:objective-three-optimal-rounding} that \emph{stochastic quantization} turns out to be optimal for $\objth$ (minimizing the worst-case variance)! When considering $\objf$, however, the situation is more challenging: in Theorem \ref{thm:addv-np-hard}, we show that computing the optimal distribution for $\objf$ (minimizing average-case variance) is NP-Hard. Given the result of Theorem \ref{thm:objective-three-optimal-rounding}, it is thus natural to fix the rounding distribution $\dasq$ both in the worst and average case settings. This directly leads to Definitions \ref{def: mdv} and \ref{def: adv} of $\objo$ and $\objt$ respectively. 



% Then, the optimization is over quantization sets $Q$. 

% The thrust of this work is in the second direction of the joint optimization over $(Q, \calD)$:
% given a rounding distribution $\dasq$, we develop efficient algorithms to find optimal and approximate quantization sets that inherently preserve inner products.
% Thus, much of this work considers the fixed rounding distribution $\dasq(w, Q)$ and optimizes the quantization set $Q$
% \bnote{I think we should clearly delineate the development of algorithms and objectives; the previous sentence is my changed version but I also left the old commented out as it's a somewhat substantive change}

% We formulate the following two corresponding objectives, and then design fast algorithms for them (the algorithmic results are outlined in Section \ref{sec: theoretical-results}).

% \newpage


% Throughout the paper, given a vector $w$, we write $\widown(Q)$ to be the largest element of $Q$ less than or equal to $w_i$ and $\wiup(Q)$ as the smallest element larger than $w_i$.

% \begin{definition}[Standard rounding distribution]
%     For a vector $w\in \mathbb{R}^{d}$ and a set $Q\subset \mathbb{R}$, we define the standard ASQ rounding distribution $\dasq(w,Q)$ to be the distribution over $Q^{d}$ where for $\bwh\sim \dasq(w,Q)$ and all $i\in [d]$, $\bwh_i=\widown(Q)$ with probability $(\wiup(Q)-w_i)/(\wiup(Q)-\widown(Q))$ and $\bwh_i=\wiup(Q)$ with probability $(w_i-\widown(Q))(\wiup(Q)-\widown(Q))$.
% \end{definition}

% It is useful to have a notion of variance of a single value $w_i$ when rounded according to a set $Q$ and $\dasq(w,Q)$.
% \begin{definition}
%     For a vector $w\in \mathbb{R}^d$ and a set $Q\subset \mathbb{R}$, let
%     \[\varasq(w_i, Q) = \var_{\bwh\sim \dasq(w,Q)}[\bwh_i] = (w_i - \widown(Q))(\wiup(Q) - w_i).\]
%     % where $\widown(Q)$ is the largest element of $Q$ less than or equal to $w_i$ and $\wiup(Q)$ is the smallest element of $Q$ larger than $w_i$.
% \end{definition}

\paragraph{Properties of $\objo$ and $\objt$.} Here, we make some simple but useful observations about the structure of the $\objo$ and $\objt$ objectives. In particular, for a fixed quantization set $Q$, we write $$\objo(w, Q) \triangleq \max_{x\in \mathbb{R}^{d}: \|x\|_2 \leq 1} \var_{\bwh\sim \dasq(w,Q)}[\langle \bwh,x \rangle]$$ to denote its $\objo$ objective cost. $\objo$ turns out to have a simple combinatorial structure. In particular, observe that
\begin{align*}
    \objo(w, Q) &= \max_{x\in \mathbb{R}^{d}: \|x\|_2 \leq 1} \left[ \var_{\bwh\sim \dasq(w,Q)}[\langle \bwh,x \rangle] \right] \\
    &= \max_{x\in \mathbb{R}^{d}: \|x\|_2 \leq 1} \left[ \sum_{i=1}^d x_i^2 \var_{\bwh\sim \dasq(w,Q)}[\bwh_i] \right] \tag{Independence of $\dasq$} \\
    &= \max_{j\in [d]} \varasq(w_j, Q).
\end{align*}
% \bnote{is ``input vector'' the best name for $x$?}
So, the worst-case input vector $x$ is the standard unit basis vector $e_i$ where $i$ is such that $\VarASQ[\bwh_i]$ is maximized. With $\lambda_i \triangleq \E_{\bx \sim \calX} [\bx_i^2]$, for a fixed quantization set $Q$, we write 
\begin{align*}
    \objt_{\calX}(w,Q) \triangleq \E_{\bx\sim \calX}[\var_{\bwh\sim \dasq(w,Q)}[\langle \bwh,\bx \rangle]] = \sum_{i=1}^d \lambda_i \cdot \varasq[\bwh_i]
\end{align*}
to denote its $\objt$ cost. The $\objt$ objective turns out to have a familiar structure. 
\begin{align*}
    \min_{Q \subset \R: |Q| \leq s} \E_{\bx \sim \calX} \left[\VarASQ \left[ \la \bwh, \bx \ra \right] \right] &= \min_{Q \subset \R: |Q| \leq s} \E_{\bx \sim \calX} \left[ \sum_{i \in [d]} \bx_i^2 \cdot \VarASQ[\bwh_i] \right] \\
    &= \min_{Q \subset \R: |Q| \leq s} \sum_{i \in [d]} \lambda_i \cdot \VarASQ[\bwh_i]
    % &= \min_{Q \subset \R: |Q| \leq s} \sum_{i \in [d]} \lambda_i \cdot (\wiup(Q) - w_i)(w_i - \widown(Q))
\end{align*}
This can be interpreted as a weighted $\MSE$ objective function! We note that this connection between quantization for average-case inner product preservation and the problem of stochastic quantization under the weighted $\MSE$ objective provides a theoretical justification for the empirical success of Adaptive Stochastic Quantization for downstream applications in ML and vector search.

% \begin{observation}
%     For any $w\in \mathbb{R}^{d}$ and $Q \subset \mathbb{R}$,
%     \[
%         \objo(w,Q) = \max_{i\in [d]} \varasq(w_i, Q).
%     \]
% \end{observation}
% \begin{proof}
%     From the definition of inner products and the fact that $\bwh_i$ are independent, we have for all $x\in \mathbb{R}^{d}$ with $\|x\|_2=1$,
%     \begin{align*}
%         &\var_{\bwh\sim \dasq(w,Q)}[\langle \bwh,x \rangle] = \var_{\bwh\sim \dasq(w,Q)}\left[\sum_{i=1}^d \bwh_i x_i\right] = \sum_{i=1}^d x_i^2 \var_{\bwh\sim \dasq(w,Q)}[\bwh_i]\\
%         =&\sum_{i=1}^d x_i^2 \varasq(w_i, Q)\leq \max_{j\in [d]} \varasq(w_j, Q) \sum_{i=1}^d x_i^2= \max_{j\in [d]} \varasq(w_j, Q).
%     \end{align*}
%     Moreover, this upper bound is achieved by the vector $x$ which is $1$ in the coordinate $i$ which achieves the maximum and $0$ elsewhere, and thus $\objo(w,Q) = \max_{i\in [d]} \varasq(w_i, Q)$.
% \end{proof}

% \onote{avoid contractions (again something the LLM can also filter out); reworded this sentence anyway but leaving commented out for prosterity and leaving this comment for our note}
% In practice, however, we oftentimes \bnote{\sout{don't}} expect to encounter the worst-case and would prefer to develop algorithms tailored to the specific data distribution we expect to see.
% In particular, if the input vectors $x$ are known to be drawn from some distribution $\calX$, we define the Average Directional Variance ($\objt$) objective as a generalization of $\objo$. Note that we use $\dasq$ as the rounding distribution.



% objective provides algorithms that convincingly outperform existing counterparts \cite{ZLKALZ17}.
% \bnote{I think this sentence is mixing algorithms and objectives a bit?}



% \onote{maybe we should add a ``our contributions'' subsection header at this point?}
% \rnote{More generally, I think this intro section might benefit from a bit more structure; it's a bit in a stream rn which could make it hard for a reader to jump to one part or another}


==> notation.tex <==
\section{Notation}

In this section, we introduce and recall notation and shorthand relevant to the technical content in the appendices. 

Recall that this work focuses on unbiased rounding distributions. For a given $w \in \R^d$ and $Q \subseteq \R$, we define
\begin{align*}
    \Omega := \{ \text{Rounding distributions } \calD : \supp(\calD) \subseteq Q^d \text{ and } \E_{\bwh \sim \calD} [\bwh] = w \}
\end{align*}

Finally, for any $v\in \mathbb{R}$, we define $\objos(w,v)$ to be the smallest value of $s$ for which $\objo(w,s)\leq v$.

We assume the input distribution has support $\supp(\calX) \subseteq \R^d$ and has finite marginal second moments. Our algorithms assume access to the marginal second moments in full precision. 


\begin{enumerate}
    \item Weights $\to \lambda_i \in [0,1]$
    \item Neighboring points $\to w^{\scriptscriptstyle \uparrow}_i(Q)$ and $w^{\scriptscriptstyle \downarrow}_i(Q)$
    \item $w$ drawn from any rounding distribution $\to \bwh$
    \item $\calD^{\scriptscriptstyle \mathsf{ASQ}}(w,Q)$. In general, rounding distribution should be $\calD$ with name of distribution in superscript 
    \item $\Var^{\scriptscriptstyle \mathsf{ASQ}}(w_i, Q)$ is shorthand for $\Var_{\bwh \sim \calD^{\scriptscriptstyle \mathsf{ASQ}}(w, Q)}[\bwh_i] = (w_i - a_i)(b_i - w_i)$
    \item Distribution over inputs $x$ $\to \calX$.
    \item Set of all rounding distributions $\to \Omega$
    \item $\mathsf{MDV}$ (max directional variance) and $\mathsf{ADV}$ (average directional variance)
    \item $\mathsf{WDDV}$ (Worst-Case Distributional Directional Variance) and $\mathsf{ADDV}$ (Average-Case Distributional Directional Variance)

    

    
\end{enumerate}




==> to-dos.tex <==
\section*{To Dos}

Krish
\begin{enumerate}
    \item Appendices 
\end{enumerate}

Nathan
\begin{enumerate}
    \item PQ vector search evals
    \item Clean up body plots
    \item Appendices
\end{enumerate}

Nice-to-haves
\begin{enumerate}
    \item CSV with full empirical results
    \item Run turbo-quant in plot 2(b)
    \item Appendix plots (decide whether to create and include)
    \item Maybe change algorithm name to PIPER
    \item 
\end{enumerate}

